Mapping Patterns for Virtual Knowledge Graphs

Virtual Knowledge Graphs (VKG) constitute one of the most promising paradigms for integrating and accessing legacy data sources. A critical bottleneck in the integration process involves the definition, validation, and maintenance of mappings that link data sources to a domain ontology. To support the management of mappings throughout their entire lifecycle, we propose a comprehensive catalog of sophisticated mapping patterns that emerge when linking databases to ontologies. To do so, we build on well-established methodologies and patterns studied in data management, data analysis, and conceptual modeling. These are extended and refined through the analysis of concrete VKG benchmarks and real-world use cases, and considering the inherent impedance mismatch between data sources and ontologies. We validate our catalog on the considered VKG scenarios, showing that it covers the vast majority of patterns present therein.

==> 4-conceptual-vs-ontologies.tex <==
\subsection{Discussion}

\davide{ADDED from CAISE. TO ADJUST}

\subsubsection{Database Schema Ontology vs.\ Domain Ontology.}
%\am{If we like the term (really?), we need a definition clarifying its meaning (and this citation: Sequeda et al, 2011). Another option is the one of using ``database schema ontology'' versus ``domain-specific ontology'' (Sparnos et al. 2012))}
Our approach based on mapping patterns puts into correspondence a database schema, together with its intended conceptualization, to a pair ``(OBDA mappings, database schema ontology)''. Following~\cite{spanos2012bringing}, with \emph{database schema ontology} we refer here to an ontology whose concepts and properties reflect the constructs of the conceptual schema, mirroring the structure of the relational database. In our approach, the database schema ontology provides a natural encoding of the conceptual schema input to each pattern, \emph{modulo} the expressivity of the \owlql language.

In real-world scenarios, however, it is usually the case that a domain ontology is developed independently from the relational data-source. The \npd and \cordis scenarios we consider here are no exception to this. This results in a misalignment between the domain ontology and the conceptual schema used for the database, which in turn results in a misalignment between the database schema ontology and the domain ontology. \emph{In our experimental evaluation we shall provide a quantitative measure over this misalignment, for both the \npd and \cordis scenarios}.
% Based on our experience, we saw that if the relational schema is reasonably well-designed, then the misalignment happens mostly at the level of the vocabulary used (e.g., different choice of class names in the target ontology as opposed to table names used in the database), rather than at the level of the structure (e.g., classes and property definitions, or hierarchies). Consequently, it is usually the case that substantial portions of the target ontology actually coincide with the database-schema ontology.


\subsubsection{Applied vs.\ Discovered Patterns.}
We start from two fundamental observations:\dl{TO REVISE}
\begin{inparaenum}[\itshape(i)]
\item a conceptual schema may have more than one admissible relational mapping, according to the applied methodology, as well as to considerations about efficiency, performance optimization, and space consumption on the final information system;
\item given the logical schema of a relational database, regardless of its normal form, more than one conceptual schema can be designed which provide (admissible) alternative representations of its domain.
\end{inparaenum}
By~\emph{(i)} and~\emph{(ii)},~\cite{arxiv-patterns}  explicitly associate a conceptual schema to each database schema in order to disambiguate among other possible conceptualizations of this latter (unlike bootstrapping-oriented approaches that can be found in the literature).

The conceptual schema of a database is typically discarded after the design and deployment phases, and therefore it is not available as input to the bootstrapping algorithm. As a result, our algorithm cannot disambiguate all the possible conceptualizations corresponding to the same database schema, but instead chooses one of them (literally, it operates according to the ``most-typical'' application of a pattern as per~\cite{arxiv-patterns}). 

\emph{To check the efficacy of this approach, we have manually analyzed the scenarios and categorized the mappings according to the schema-driven mapping patterns that were actually used in such scenarios}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> macros-style.tex <==

\makeatletter
\g@addto@macro\normalsize{%
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-10pt}
\setlength\abovedisplayskip{3pt}
\setlength\belowdisplayskip{3pt}
\setlength\abovedisplayshortskip{3pt}
\setlength\belowdisplayshortskip{3pt}
}
\makeatother


==> macros-theorems.tex <==
%% fancy theorem environments

\usepackage[thmmarks,amsmath,thref,hyperref]{ntheorem}
% thref allows for extended labeling - ntheorem must be loaded after babel
% ntheorem must be loaded after amsmath
% \usepackage{hyperref} must appear before the first use of \newtheorem

\theorempreskip{1pt}
\theorempostskip{1pt}

% Adjust use of counters as needed
% \newcounter{thmcnt}
% \setcounter{thmcnt}{1}
% %\numberwithin{thmcnt}{section}
% \newcounter{thmcnt1} \setcounter{thmcnt1}{1}
% \newcounter{thmcnt2} \setcounter{thmcnt2}{1}
% \newcounter{thmcnt3} \setcounter{thmcnt3}{1}
% \newcounter{thmcnt4} \setcounter{thmcnt4}{1}
% \newcounter{thmcnt5} \setcounter{thmcnt5}{1}
% \newcounter{thmcnt6} \setcounter{thmcnt6}{1}
% \newcounter{thmcnt7} \setcounter{thmcnt7}{1}

% Used for all numbered theorem-like environments
% Default settings
% \theoremstyle{plain}
% \theoremheaderfont{\normalfont\bfseries}
% \theorembodyfont{\itshape}
% \theoremseparator{}
% \theorempreskip{\topsep}
% \theorempostskip{\topsep}
% \theoremindent 0cm
% \theoremnumbering{arabic}
% \theoremsymbol{}

% For theorems
\let\theorem\relax
\let\proposition\relax
\let\lemma\relax
\let\corollary\relax
\theoremseparator{.}
\theorembodyfont{\itshape}
\theoremsymbol{\mbox{$\triangleleft$}} % \mbox is needed!
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

% For definitions
\let\definition\relax
\theoremseparator{.}
\theorembodyfont{\upshape}
\theoremsymbol{\mbox{$\triangleleft$}} % \mbox is needed!
%\theoremsymbol{\mbox{\qedboxfull}}
\newtheorem{definition}[theorem]{Definition}

% For examples
\let\remark\relax
\let\example\relax
\theorembodyfont{\upshape}%\small
\theoremsymbol{\mbox{$\triangleleft$}} % \mbox is needed!
%\theoremsymbol{\mbox{\qedboxfull}}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

% For proofs
\let\proof\relax
\theoremstyle{nonumberplain}
%\theoremheaderfont{\scshape}
\theoremheaderfont{\itshape}
\theorembodyfont{\upshape}%\small
%\theoremsymbol{\mbox{$\square$}} % \mbox is needed!
\theoremsymbol{\mbox{$\dashv$}} % \mbox is needed!
\newtheorem{proof}{Proof}

\qedsymbol{\ensuremath{\dashv}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> tables/data-driven-clustering.tex <==
\begin{table}
  \caption{Clustering Patterns (Data-driven). $\zeta$, $\xi$ are two possibly
   \emph{not-injective} functions}
  \label{tab:clustering-patterns}
  \begin{tabularx}{\textwidth}{lcXl@{}}
    \toprule
    \textsc{E-R diagram}
    & \begin{tabular}{@{}l}
      \textsc{Schema Level}\\\midrule \textsc{Data Level}
    \end{tabular}~~~~
    & \textsc{Mapping pattern}
    & \textsc{Ontology}\\
    \midrule
    \multicolumn{4}{c}{\textbf{Clustering Entity to Class (CE2C)}}\\
    \begin{minipage}{0.85\erw}
      \begin{center}
        \includegraphics[width=0.3\textwidth]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
          \sB \subseteq \sK\cup\sA,\\
          \partition_\D(\sB,E)
        \end{array}
        $
      \end{center}
    \end{minipage}
    & $\begin{array}{l}
         T_E(\sK, \sA), \\
         \key[T_E]{\sK} \\
         \sB \subseteq \sK\cup\sA,\\
         \partition_\D(\sB,E) \\
         \midrule
         \{V_{E_\sv}(\sK,\sA) = \\
         \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
    & $\begin{array}{@{}l@{~}l}
           \{s: & \sigma_{\sB = \sv}(T_E) \\
           ~~t: & C_E^{\sv}(\iri_E(\sK))\}_{\sv \in \pi_{\sB} (T_E)}
         \end{array}$
    & $\{C_E^{\sv} \sqsubseteq C_E \}_{\sv \in \pi_{\sB} (T_E)}$\\
    \midrule
    \multicolumn{4}{c}{\textbf{Clustering Entity to Data Property (CE2D)}}\\
    \begin{minipage}{0.85\erw}
      \begin{center}
        \includegraphics[width=0.3\textwidth]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
          \sB \subseteq \sK\cup\sA,\\
          \partition_\D(\sB,E)
        \end{array}
        $
      \end{center}
    \end{minipage}
    & $\begin{array}{l}
         T_E(\sK, \sA), \\
         \key[T_E]{\sK} \\
           \sB \subseteq \sK\cup\sA,\\
           \partition_\D(\sB,E) \\
         \midrule
         \{V_{E_{\xi(\sv)}}(\sK,\sA) = \\
         \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
    & $\begin{array}{@{}l@{~}l}
           \{s: & \sigma_{\sB = \sv}(T_E) \\
           ~~t: & d_{\sB}(
           \begin{array}[t]{@{}l}
             \iri_E(\sK),\\
             \xi(\sv)) \}_{\sv \in \pi_{\sA} (T_E)}
           \end{array}
         \end{array}$
    & $\exists d_{\sB} \sqsubseteq C_E$\\
    \midrule
    \multicolumn{4}{c}{\textbf{Clustering Entity to Object Property (CE2O)}}\\
    \begin{minipage}{0.85\erw}
      \begin{center}
        \includegraphics[width=0.3\textwidth]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
          \sB \subseteq \sK\cup\sA,\\
          \partition_\D(\sB,E)
        \end{array}
        $
      \end{center}
    \end{minipage}
    & $\begin{array}{l}
         T_E(\sK, \sA), \\
         \key[T_E]{\sK} \\
         \sB \subseteq \sK\cup\sA,\\
         \partition_\D(\sB,E) \\
         \midrule
         \{V_{E_\sv}(\sK,\sA) = \\
         \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
    & $\begin{array}{@{}l@{~}l}
           \{s: & \sigma_{\sB = \sv}(T_E) \\
         ~~t: & r_{\sB}(
         \begin{array}[t]{@{}l}
           \iri_E(\sK), \\
           \iri_{\sB}(\zeta(\sv))) \}_{\sv \in \pi_{\sB} (T_E)}
         \end{array}
       \end{array}$
    & $\exists r_{\sB} \sqsubseteq C_E$\\
    \bottomrule
  \end{tabularx}
\end{table}

\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

==> tables/discarded-patterns.tex <==
\endinput

    \multicolumn{4}{c}{\textbf{Data Entity with Merged 1-N Relationship and
        Entity with Relationship (DR1NRm)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR1NRm.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK_E},\sA_E,\sK\tikz\coordinate(kF);_F)$};
        \node[below=of e.south west,anchor=north west] (s)
          {$T_S(\pk{\sK\tikz\coordinate(kSG);_{SG},
            \sK\tikz\coordinate(kSF);_{SF}})$};
        \node[below=of s.south west,anchor=north west] (g)
          {$T_G(\pk{\sK\tikz\coordinate(kG);_G},\sA_G)$};
        \draw[->] ($(kSG)+(0.7mm,-\doffset)$) -- ($(kG)+(0,\uoffset)$);
        % \draw[->] ($(kSG)-(0,\doffset)$) |- ($(kSG)-(0,\ddoffset)$) -|
        %  ($(kG)+(0,\uoffset)$);
        \draw[->] ($(kSF)+(0,\uoffset)$) |- ($(kSF)+(0,\uuoffset)$) -|
        ($(kF)-(0,\doffset)$);
      \end{tikzpicture}\\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (ve)
        {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) = \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of ve.south west,anchor=north west] (vr)
        {$V_R(\pk{\sK\tikz\coordinate(kRE);_E,\sK\tikz\coordinate(kRF);_F}) =
          \pi_{\sK_E,\sK_F} (T_E)$};
        \node[below=of vr.south west,anchor=north west] (vf)
        {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
        ($(kF)+(0,\uoffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s{:} & T_E \\
      t{:} & C_F(\iri_F(\sK_F)), \\
           & \{d_A(\iri_F(\sK_F),A)\}_{A \in \sK_F}, \\
           & p_R(\iri_E(\sK_E),\iri_F(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
      \{\exists d_A \sqsubseteq C_E\}_{A \in \sK_E\cup\sA_E}\\
      \{\exists d_A \sqsubseteq C_F\}_{A \in \sK_F}\\
      \exists p_R \sqsubseteq C_E \\
      \exists p_R^- \sqsubseteq C_F
    \end{array}$
    \\

    \midrule
%
\midrule
    % \multicolumn{4}{c}{\textbf{Data Entity with No Pkey, Cardinality Preserving (DENoPKeyBag)}}\\
    % \begin{minipage}{\erw}
    %   \begin{center}
    %     \includegraphics[scale=\erscale]{img/er-DENoKeyBag}
    %   \end{center}
    % \end{minipage}
    % & $\begin{array}{l}
    %      T_E(\sA) \\
    %      \bottomrule
    %      V_{E}(rid,\sA) = \\
    %      \quad \pi_{\texttt{rid}, \sA} (T_E) \\
    %      \key[V_E]{rid}
    %    \end{array}$
    % & $\begin{array}{@{}l@{~}l}
    %        \{s: & \sigma_{\sB = \sv}(T_R) \\
    %      ~~t: & p_R^{\sv}(
    %      \begin{array}[t]{@{}l}
    %        \iri_E(\sK_{RE}), \\
    %        \iri_F(\sK_{RF})) \}_{\sv \in \pi_{\sB} (T_R)}
    %      \end{array}
    %    \end{array}$
    %    & $\begin{array}{l}
    %         \{p_R^{\sv} \sqsubseteq p_R \}_{\sv \in \pi_{\sB} (T_R)}
    %       \end{array}$\\

\midrule
                             \multicolumn{4}{c}{\textbf{Clustering Relationship to Object Property (CR2O)}\todo{REMOVE: once a relationship is handled, we want no further patterns to be applicable on it. Fullstop. Otherwise, I should create a view for each alignment on relationship, and this explodes immediately (especially with SRm and SRma, where a complete view for the relationship should be created from scratch)}}\\
                             \begin{minipage}{\erw}
                               \begin{center}
                                 \includegraphics[scale=\erscale]{img/er-CR2O.pdf}
                                 \smallskip
                                 $\begin{array}{c}
                                    \sB \subseteq \sK_{RE}\cup\sK_{RF}\\
                                    \partition_\D(\sB,R)
                                  \end{array}
                                  $
                                  partitions to relationships
                                \end{center}
                              \end{minipage}
                              & $\begin{array}{l}
                                   T_R(\pk{\sK_{RE},\sK_{RF}}), \\
                                   \sB \subseteq \sK_{RE}\cup\sK_{RF}\\
                                   \partition_\D(\sB,R) \\
                                 \end{array}$
                                 & $\left\{
                                   \begin{array}{l@{~}l}
                                     s: & \sigma_{\mathfrak{p}}(T_R) \\
                                     t: & p_R^{\mathfrak{p}}(
                                          \begin{array}[t]{@{}l}
                                            \iri_{C_E}(\sK_{RE}), \\
                                            \iri_{C_F}(\sK_{RF}))
                                          \end{array}
                                   \end{array}\!\!\!\!
                                 \right\}_{\mathfrak{p} \in \partition_\D(\sB,E)}$
                                 &
                                 \hspace{.7em}$\{p_R^{\mathfrak{p}} \sqsubseteq p_R \}_{\mathfrak{p} \in \partition_\D(\sB,E)}$ \\[4em]
                                 \multicolumn{4}{l}{\footnotesize
                                   \begin{minipage}{1.46\textwidth}
                                     In case of $(\_,1)$ cardinality on role $R_E$ (resp., $R_F$), the primary key for $T_R$ is restricted to the attributes $\sK_{RE}$ (resp., $\sK_{RF}$). The pattern extends to N-ary relationships by proceeding similarly to pattern \pat{SRR}.
                                   \end{minipage}
                                 } \\

\midrule
      \multicolumn{4}{c}{\textbf{Schema Weak-Entity with Alignment (SEwa/DEwa)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SEwa.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (f)
          {$T_F(\pk{\sK_F},\sU\tikz\coordinate(kF);_F,\sA_F)$};
        \node[below=of f.south west,anchor=north west] (e)
          {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kEF);_{EF}},\sA_E)$};
        \draw[->] ($(kEF)+(0,\uoffset)$) |- ($(kEF)+(0,\uoffset)$) -|
          ($(kF)-(0,\doffset)$);
          \node[right of=f, xshift=2cm] {$\key[T_F]{\sU_F}$} ;
      \end{tikzpicture}
    \end{tabular}
    & $\begin{array}{l@{~}l}
        s{:} & T_E \Join_{\sK_{EF} = \sU_{F}} T_F \\
        t{:} & C_E(\iri_{E}(\sK_E, \sK_{EF})), \\
             & \{d_A(\iri_E(\sK_E, \sK_{EF}),A)\}_{A \in \sK_E \cup \sA_E} \\
             & p_{EF}(\iri_{E}(\sK_E, \sK_{EF}),\iri_{C_F}(\sK_{F}))
      \end{array}$
    & $\begin{array}{l@{}}
         \left\{\begin{array}{l}
                  \delta(d_A) \sqsubseteq C_E, \\
                  \rho(d_A) \sqsubseteq \mu(\tau(A))
                \end{array}
         \right\}_{A \in \sK_E\cup\sA_E} \\
        \exists p_{EF} \equiv C_E \\
        \exists p_{EF}^- \sqsubseteq C_F
      \end{array}$
      \\[5ex]
      \multicolumn{4}{l}{\small
        \begin{minipage}{1.48\textwidth}
          \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
          Cardinality constraints are handled similarly as for \pat{SR}, with the difference that now the constraints now involve $U_F$ and $K_{EF}$.
        \end{minipage}
      }\\

\multicolumn{4}{c}{\textbf{Schema/Data Relationship with Merging (SRma/DRma)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRma.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (f)
          {$T_F(\pk{\sK_F}, \sU\tikz\coordinate(kF);_{F}, \sA_F)$};
        \node[below=of f.south west,anchor=north west] (e)
          {$T_E(\pk{\sK_E},\sK\tikz\coordinate(kEF);_{EF},\sA_E)$};
        \draw[->] ($(kEF)+(0,\uoffset)$) |- ($(kEF)+(0,\uuoffset)$) -|
        ($(kF)-(0,\doffset)$);
        \node[right of=f, xshift=2cm] {$\key[T_F]{\sU_F}$};
      \end{tikzpicture}
    \end{tabular}
    & $\begin{array}{l@{~}l}
        s{:} & T_E \Join_{\sK_{EF} = \sU_{F}} T_F \\
        t{:} & p_{EF}(\iri_{C_E}(\sK_E),\iri_{C_F}(\sK_{F}))
      \end{array}$
    & $\begin{array}{l@{}}
        \exists p_{EF} \sqsubseteq C_E \\
        \exists p_{EF}^- \sqsubseteq C_F
      \end{array}$
      \\[5ex]
      \multicolumn{4}{l}{\small
       \begin{minipage}{1.48\linewidth}
         \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}

         Cardinality constraints are handled similarly as for \pat{SR}, with the difference that now the constraints now involve $U_F$ and $\sK_{EF}$.
       \end{minipage}
     } \\
%
\midrule
    % \multicolumn{4}{c}{\textbf{Data Entity with No Pkey, Cardinality Preserving (DENoPKeyBag)}}\\
    % \begin{minipage}{\erw}
    %   \begin{center}
    %     \includegraphics[scale=\erscale]{img/er-DENoKeyBag}
    %   \end{center}
    % \end{minipage}
    % & $\begin{array}{l}
    %      T_E(\sA) \\
    %      \bottomrule
    %      V_{E}(rid,\sA) = \\
    %      \quad \pi_{\texttt{rid}, \sA} (T_E) \\
    %      \key[V_E]{rid}
    %    \end{array}$
    % & $\begin{array}{@{}l@{~}l}
    %        \{s: & \sigma_{\sB = \sv}(T_R) \\
    %      ~~t: & p_R^{\sv}(
    %      \begin{array}[t]{@{}l}
    %        \iri_E(\sK_{RE}), \\
    %        \iri_F(\sK_{RF})) \}_{\sv \in \pi_{\sB} (T_R)}
    %      \end{array}
    %    \end{array}$
    %    & $\begin{array}{l}
    %         \{p_R^{\sv} \sqsubseteq p_R \}_{\sv \in \pi_{\sB} (T_R)}
    %       \end{array}$\\

\multicolumn{4}{c}{\textbf{Data Entity with Merged 1-N Relationship and
        Entity with Relationship (DR1NRm)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR1NRm.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK_E},\sA_E,\sK\tikz\coordinate(kF);_F)$};
        \node[below=of e.south west,anchor=north west] (s)
          {$T_S(\pk{\sK\tikz\coordinate(kSG);_{SG},
            \sK\tikz\coordinate(kSF);_{SF}})$};
        \node[below=of s.south west,anchor=north west] (g)
          {$T_G(\pk{\sK\tikz\coordinate(kG);_G},\sA_G)$};
        \draw[->] ($(kSG)+(0.7mm,-\doffset)$) -- ($(kG)+(0,\uoffset)$);
        % \draw[->] ($(kSG)-(0,\doffset)$) |- ($(kSG)-(0,\ddoffset)$) -|
        %  ($(kG)+(0,\uoffset)$);
        \draw[->] ($(kSF)+(0,\uoffset)$) |- ($(kSF)+(0,\uuoffset)$) -|
        ($(kF)-(0,\doffset)$);
      \end{tikzpicture}\\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (ve)
        {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) = \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of ve.south west,anchor=north west] (vr)
        {$V_R(\pk{\sK\tikz\coordinate(kRE);_E,\sK\tikz\coordinate(kRF);_F}) =
          \pi_{\sK_E,\sK_F} (T_E)$};
        \node[below=of vr.south west,anchor=north west] (vf)
        {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
        ($(kF)+(0,\uoffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s{:} & T_E \\
      t{:} & C_F(\iri_F(\sK_F)), \\
           & \{d_A(\iri_F(\sK_F),A)\}_{A \in \sK_F}, \\
           & p_R(\iri_E(\sK_E),\iri_F(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
      \{\exists d_A \sqsubseteq C_E\}_{A \in \sK_E\cup\sA_E}\\
      \{\exists d_A \sqsubseteq C_F\}_{A \in \sK_F}\\
      \exists p_R \sqsubseteq C_E \\
      \exists p_R^- \sqsubseteq C_F
    \end{array}$
    \\

    \midrule
    

Prima di rimuovere le viste per le relationships:

\multicolumn{4}{c}{\textbf{Data Entity with Merged 1-N Relationship and
      Entity (DR1Nm)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR1Nm.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
        T_E(\pk{\sK_E},\sA_E,\sK_F,\sA_F)\\[1ex]
        \fd[T_E]{\sK_F}{\sA_F}\\
      \end{array}$\\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (ve)
          {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) = \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of ve.south west,anchor=north west] (vr)
          {$V_R(\pk{\sK\tikz\coordinate(kRE);_E},\sK\tikz\coordinate(kRF);_F) =
           \pi_{\sK_E,\sK_F} (T_E)$};
        \node[below=of vr.south west,anchor=north west] (vf)
          {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
          ($(kF)+(0,\uoffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s_1{:} & V_E \\
       t_1{:} & C_E(\iri_E(\sK_E)), \\
             & \{d_A(\iri_E(\sK_E),A)\}_{A \in \sK_F\cup\sA_E}, \\
       s_2{:} & V_F \\
       t_2{:} & C_F(\iri_F(\sK_F)), \\
             & \{d_A(\iri_F(\sK_F),A)\}_{A \in \sK_F\cup\sA_F}, \\
       s_3{:} & V_R \\
       t_3{:} &  p_R(\iri_E(\sK_E),\iri_F(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
       \left\{
       \begin{array}{l}
         \delta(d_A) \sqsubseteq C_F, \\
         \rho(d_A) \sqsubseteq \mu(\tau(A))
       \end{array}
         \right\}_{A \in \sK_F\cup\sA_F}\\
      \exists p_R \sqsubseteq C_E \\
      \exists p_R^- \sqsubseteq C_F
    \end{array}$
    \\
    \midrule
        \multicolumn{4}{c}{\textbf{Data 1-1 Relationship with Merging (DR11m)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR11m.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
        T_E(\pk{\sK_E},\sA_E,\sK_F,\sA_F) \\
        \key[T_E]{\sK_F}
      \end{array}$\\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (vr)
          {$V_R(\pk{\sK\tikz\coordinate(kRE);_E},\sK\tikz\coordinate(kRF);_F) =
           \pi_{\sK_E,\sK_F} (T_E)$};
        \node[above=of vr.north west,anchor=south west] (ve)
          {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) =
           \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of vr.south west,anchor=north west] (vf)
          {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \draw[<->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
          ($(kF)+(0,\uoffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
       s_1{:} & V_E \\
       t_1{:} & C_E(\iri_E(\sK_E)), \\
              & \{d_A(\iri_E(\sK_E),A)\}_{A \in \sK_E\cup\sA_E}, \\
      s_2{:} & V_F \\
      t_2{:} & C_F(\iri_F(\sK_F)), \\
           & \{d_A(\iri_F(\sK_F),A)\}_{A \in \sK_F\cup\sA_F}, \\
       s_3{:} & V_R \\
       t_3{:} &  p_R(\iri_E(\sK_E),\iri_F(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
       \left\{
       \begin{array}{l}
         \delta(d_A) \sqsubseteq C_F \\
         \rho(d_A) \sqsubseteq \mu(\tau(A)) \\
       \end{array}
         \right\}_{A \in \sK_F\cup\sA_F} \\
      \exists p_R \equiv C_E \\
      \exists p_R^- \sqsubseteq C_F
    \end{array}$
    \\


Version of SRa with view 

\multicolumn{4}{c}{\textbf{Schema/Data Relationship with Identifier Alignment
        (SRa/DRa)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRa.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK_F},\sU\tikz\coordinate(uF);_F,\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
              \sU\tikz\coordinate(kUF);_{RF}})$};
        \node[right=of r] (k) {$\unique[R_F]{\sU_F}$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kUF)+(0,\uoffset)$) |- ($(kUF)+(0,\uuoffset)$) -|
          ($(uF)-(0,\doffset)$);
        \end{tikzpicture}\\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
        {$V_R(\pk{\sK\tikz\coordinate(kRE);_{RE},\sK\tikz\coordinate(kRF);_{F}}) = T_R \Join_{\sU_{RF}=\sU_F} T_F$ };
        \node[right=of e.east,anchor=west] (r) {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sU_F,\sA_F)$};
        \node[below=of r.south, yshift=-.5cm,xshift=-.2cm] (k) {$\unique[R_F]{\sU_F}$};
        \draw[->] ($(kRE)+(0,\uoffset)$) |- ($(kRE)+(0,\uuoffset)$) -| ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -| ($(kF)-(0,\doffset)$);
        \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s{:} & V_R\\
      t{:} & p_R(\iri_{C_E}(\sK_{RE}),\iri_{C_F}(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
%      \{\exists d_A \sqsubseteq C_F \\
%      ~~\}_{A \in \sK_F\cup\sU_F\cup\sA_F} \\
      \exists p_R \sqsubseteq C_E \\
      \exists p_R^- \sqsubseteq C_F
     \end{array}$\\
     \multicolumn{4}{l}{\footnotesize
       \begin{minipage}{1.48\textwidth}
         \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
         Cardinality constraints are handled similarly as for \pat{SR}, with the difference that now the constraints now also involve $U_R$ and that if the participation on role $R_F$ is mandatory (i.e., $(1,\_)$), then the unique constraint becomes a key constraint.
       \end{minipage}
     } \\
    \midrule

% \midrule
    % \multicolumn{4}{c}{\textbf{Schema/Data Hierarchy with Advanced Alignment (SHaa/DHaa)}}\\
    % \begin{minipage}{\erw}
    %   \begin{center}
    %      \includegraphics[scale=\erscale]{img/er-SHaa.pdf}\\
    %      {\footnotesize $\sK_{E}$ in $F$ is a constant \texttt{c},\\[-.5ex]
    %        $\sK_{EF}$ alone identifies $F$.
    %      }
    %    \end{center}
    %  \end{minipage}
    %  &
    %  \begin{tabular}{l}
    %    \begin{tikzpicture}[dbpicture]
    %      \node (e)
    %        {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kEF);_{EF}},\sA_E)$};
    %      \node[below=of e.south west,anchor=north west] (f)
    %      {$T_F(\pk{\sK\tikz\coordinate(kF);_{F}},\sA_F)$};
    %      \draw[->, dashed] ($(kF)+(0,\uoffset)$) |- ($(kF)+(0,\uuoffset)$) -| ($(kEF)-(0,\doffset)$);
    %    \end{tikzpicture}
    %  \end{tabular}
    %  &
    %    $\begin{array}{l@{~}l}
    %      s{:} & \pi_{\texttt{c}, \sK_{F}}(T_F) \\
    %      t{:} & C_F(\iri_E(\texttt{c}, \sK_{F})), \\
    %           & \{d_A(\iri_E(\texttt{c},\sK_{F}),A)\}_{A \in \sA_F}
    %     \end{array}$
    %  &
    %    $\begin{array}{l@{}}
    %       C_F \sqsubseteq C_E \\
    %       \{\exists d_A \sqsubseteq C_F \}_{A \in \sA_F}
    %    \end{array}$
    %    \\~\\[-1ex]
    %    \multicolumn{4}{l}{\footnotesize
    %    \begin{minipage}{1.48\linewidth}
    %      $\sK_{E}$ is not inherited by the child table, because it is a constant value \texttt{c}. The dependency between $T_F$ and $T_E$ is an inclusion dependency, rather than a foreign key dependency.
    %    \end{minipage}
    %  }\\

==> tables/ontology-mapping.tex <==
% Entity $E$ of attributes $\sA$ and primary identifier $\sK \subseteq \sA$
\begin{table}[t!]
  \caption{Ontology-mapping Functions}
  \label{tab:ontology-mapping-functions}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabularx}{1.4\textwidth}{lcXl@{}}
    \toprule
    \textsc{E-R diagram} & \textsc{DB schema} & \textsc{Mapping pattern} & \textsc{Ontology}\\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Entity (SE/DE)}}\\
    \begin{minipage}{\erw}
      \centerline{\includegraphics[scale=\erscale]{img/er-SE.pdf}}
    \end{minipage}
    &
    % \begin{tabular}{l}
    %   \begin{tikzpicture}[dbpicture]
    %     \node (e) {$T_E(\pk{\sK},\sA)$};
    %   \end{tikzpicture}
    % \end{tabular}
    $T_E(\pk{\sK},\sA)$
    &
    $\begin{array}{l@{~}l}
      s{:} & T_E \\
      t{:} & C_E(\iri_E(\sK)), \\
           & \{d_A(\iri_E(\sK),A)\}_{A \in \sK\cup\sA}
    \end{array}$
    &
    $\begin{array}{l@{}}
      \{\exists d_A \sqsubseteq C_E \}_{A \in \sK\cup\sA}
    \end{array}$
    \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Relationship (SR/DR)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SR.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
              \sK\tikz\coordinate(kRF);_{RF}})$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
        s{:} & T_R \\
        t{:} & p_R(\iri_E(\sK_{RE}),\iri_F(\sK_{RF}))
      \end{array}$
    &
      $\begin{array}{l@{}}
        \exists p_R \sqsubseteq C_E \\
        \exists p_R^- \sqsubseteq C_F
       \end{array}$\\
       \multicolumn{4}{l}{\footnotesize
         In case of $(\_,1)$ cardinality on role $R_E$ (resp., $R_F$), the primary key for $T_R$ is restricted to the attributes $\sK_{RE}$ (resp., $\sK_{RF}$).
       } \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Relationship with Merging (SRm/DRm)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRm.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of f.south west,anchor=north west] (e)
          {$T_E(\pk{\sK_E},\sK\tikz\coordinate(kEF);_{EF},\sA_E)$};
        \draw[->] ($(kEF)+(0,\uoffset)$) |- ($(kEF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    & $\begin{array}{l@{~}l}
        s{:} & T_E \\
        t{:} & p_{EF}(\iri_E(\sK_E),\iri_F(\sK_{EF}))
      \end{array}$
    & $\begin{array}{l@{}}
        \exists p_{EF} \sqsubseteq C_E \\
        \exists p_{EF}^- \sqsubseteq C_F
      \end{array}$
    \\
    \midrule
    % \multicolumn{4}{c}{\textbf{Schema Entity with Weak Identification (SEw)}}\\
    % \begin{minipage}{\erw}
    %   \includegraphics[scale=\erscale]{img/er-SEw.pdf}
    % \end{minipage}
    % &
    % \begin{tabular}{l}
        %         \begin{tikzpicture}[dbpicture]
    %     \node (f)
    %       {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
    %     \node[below=of f.south west,anchor=north west] (e)
    %       {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kRF);_{RF}},\sA_E)$};
    %     \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
    %       ($(kF)-(0,\doffset)$);
    %   \end{tikzpicture}
    % \end{tabular}
    % &
    % $\begin{array}{l@{~}l}
    %   s{:} & T_E \\
    %   t{:} & C_E(\iri_E(\sK_E,\sK_{RF})), \\
    %        & \{ d_A(\iri_E(\sK_E,\sK_{RF}), A) \\
    %        & ~~\}_{A \in \sK_E \cup \sK_{RF} \cup \sA_E}, \\
    %        & p_R(\iri_E(\sK_E,\sK_{RF}),\iri_F(\sK_{RF}))
    % \end{array}$
    % &
    % $\begin{array}{l@{}}
    %   \{\exists d_A \sqsubseteq C_E \\
    %   ~~\}_{A \in \sK_E\cup\sA_E} \\
    %   \exists p_R \sqsubseteq C_E \\
    %   \exists p_R^- \sqsubseteq C_F
    % \end{array}$\\
    % \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Reified Relationship (SRR/DRR)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRR.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      $\sK_R:=\sK_{RE}\cup\sK_{RF}\cup\sK_{RG}$\\
      \begin{tikzpicture}[dbpicture]
        \node (g)
          {$T_G(\pk{\sK\tikz\coordinate(kG);_G},\sA_G)$};
        \node[below=of g] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
            \sK\tikz\coordinate(kRF);_{RF},
            \sK\tikz\coordinate(kRG);_{RG}},
           \sA_R)$};
        \node[below=of r.south west,anchor=north west] (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \draw[->] ($(kRE)-(0,\doffset)$) -- ($(kE)+(0,\uoffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
          ($(kF)+(0,\uoffset)$);
        \draw[->] ($(kRG)+(0,\uoffset)$) |- ($(kRG)+(0,\uuoffset)$) -|
          ($(kG)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s{:} & T_R\\
      t{:} & C_R(\iri_R(\sK_R)), \\
      %    & \{d_A(\iri_R(\sK_R), A)\}_{A \in \atts(T_R)}, \\
           & \{d_A(\iri_R(\sK_R), A)\}_{A \in \sK_R\cup\sA_R}, \\
           & p_{RE}(\iri_R(\sK_R), \iri_E(\sK_{RE})), \\
           & p_{RF}(\iri_R(\sK_R), \iri_F(\sK_{RF})), \\
           & p_{RG}(\iri_R(\sK_R), \iri_G(\sK_{RG}))
    \end{array}$
    &
    $\begin{array}{l@{}}
      \exists p_{RE} \sqsubseteq C_R \\
      \exists p_{RE}^- \sqsubseteq C_E \\
      \exists p_{RF} \sqsubseteq C_R \\
      \exists p_{RF}^- \sqsubseteq C_F \\
      \exists p_{RG} \sqsubseteq C_R \\
      \exists p_{RG}^- \sqsubseteq C_G \\
      \{\exists d_A^- \sqsubseteq C_R\}_{A \in \sK_R\cup\sA_R}
     \end{array}$\\
     \multicolumn{4}{l}{\footnotesize
       \begin{minipage}{1.37\linewidth}
         \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
         ~\smallskip
         \pat{SRR} applies whenever there are three or more participating roles, or when the relationship has attributes.
         \begin{compactitem}
         \item If $R$ is identified by a strict subset $X$ of the participating roles, then the primary key of table $T_R$ (and the corresponding set of attributes $\sK_R$) is restricted to the foreign keys corresponding to the roles in $X$.
         For instance, if $R$ is identified by roles $R_E$ and $R_G$, then the primary key of $T_R$ (and the corresponding set of attributes $\sK_R$) is $\sK_{RE} \cup \sK_{RG}$.

       \item If one of the foreign keys is to a non-primary key set of attributes, the object property relative to that foreign key is dealt with as in \pat{SRa}.
       \end{compactitem}
       \end{minipage}
   } \\
   \midrule
   \multicolumn{4}{c}{\textbf{Schema/Data Entity Hierarchy (SEH/DEH)}}\\
    \begin{minipage}{\erw}
      \centerline{\includegraphics[scale=\erscale]{img/er-SH.pdf}}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_{FE}},\sA_F)$};
        \draw[->] ($(kF)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
        s{:} & T_F \\
        t{:} & C_F(\iri_E(\sK_{FE})), \\
             & \{d_A(\iri_E(\sK_{FE}),A)\}_{A \in \sA_F}
       \end{array}$
    &
      $\begin{array}{l@{}}
         C_F \sqsubseteq C_E \\
         \{\exists d_A^- \sqsubseteq C_F \}_{A \in \sA_F}
      \end{array}$
      \\
      \midrule
      % \multicolumn{4}{c}{\textbf{Schema/Data Relationship Hierarchy (SRH/DRH)}}\\
      % TODO \\
      % \midrule
          \multicolumn{4}{c}{\textbf{Clustering Entity to Class (CE2C)}}\\
    \begin{minipage}{\erw}
      \begin{center}
        \includegraphics[scale=\erscale]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
          \sB \subseteq \sK\cup\sA,\\
          \partition_\D(\sB,E)
        \end{array}
        $
      \end{center}
    \end{minipage}
    & $\begin{array}{l}
         T_E(\sK, \sA) \\
         \key[T_E]{\sK} \\
         \sB \subseteq \sK\cup\sA \\
         \partition_\D(\sB,E) \\
         \bottomrule
         \{V_{E_{\sv}}(\sK,\sA) = \\
         \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
    & $\begin{array}{@{}l@{~}l}
         \{s: & \sigma_{\sB = \sv}(T_E) \\
         ~~t: & C_E^{\sv}(\iri_E(\sK))\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
       & $\begin{array}{l}
            \{C_E^{\sv} \sqsubseteq C_E \}_{\sv \in \pi_{\sB} (T_E)}
          \end{array}$\\
    \midrule
    \multicolumn{4}{c}{\textbf{Clustering Entity to Data/Object Property (CE2D/CE2O)}}\\
    \begin{minipage}{\erw}
      \begin{center}
        \includegraphics[scale=\erscale]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
          \sB \subseteq \sK\cup\sA,\\
          \partition_\D(\sB,E)
        \end{array}
        $
      \end{center}
    \end{minipage}
    & $\begin{array}{l}
         T_E(\sK, \sA) \\
         \key[T_E]{\sK} \\
           \sB \subseteq \sK\cup\sA \\
           \partition_\D(\sB,E) \\
         \bottomrule
         \{V_{E_{\sv}}(\sK,\sA) = \\
         \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
       \end{array}$
    & \multicolumn{2}{l}{
      $
      \begin{array}{l@{\quad~~~}l@{\hspace{1.55cm}}}
        \begin{array}{@{}l@{~}l}
          \{s: & \sigma_{\sB = \sv}(T_E) \\
            ~~t: & d_{\sB}(\iri_E(\sK), \xi(\sv)) \}_{\sv \in \pi_{\sA} (T_E)}
         \end{array}
         & \hspace{.49cm}\exists d_{\sB} \sqsubseteq C_E\\
         \midrule
         \begin{array}{@{}l@{~}l}
           \{s: & \sigma_{\sB = \sv}(T_E) \\
           ~~t: & p_{\sB}(\iri_E(\sK), \iri_{\sv}(\sv)) \}_{\sv \in \pi_{\sB} (T_E)}
         \end{array}
         & \hspace{.49cm} \exists p_{\sB} \sqsubseteq C_E
       \end{array}$
    }\\
    % \midrule
    % \multicolumn{4}{c}{\textbf{Clustering Relationship to Object Property
    %   (CR2O)}}\\
    % \begin{minipage}{\erw}
    %   \begin{center}
    %     \includegraphics[scale=\erscale]{img/er-CR2O.pdf}
    %     \smallskip
    %     $\begin{array}{c}
    %        \sB \subseteq \sK_{RE}\cup\sK_{RF},\\
    %        \partition_\D(\sB,R)
    %     \end{array}
    %     $
    %   \end{center}
    % \end{minipage}
    % & $\begin{array}{l}
    %      T_R(\sK_{RE},\sK_{RF}), \\
    %      \sB \subseteq \sK_{RE}\cup\sK_{RF}\\
    %      \partition_\D(\sB,R) \\
    %      \bottomrule
    %      \{V_{R_{\sv}}(\sK_{RE},\sK_{RF}) = \\
    %      \quad \sigma_{\sB = \sv}(T_R)\}_{\sv \in \pi_{\sB} (T_R)}
    %    \end{array}$
    % & $\begin{array}{@{}l@{~}l}
    %        \{s: & \sigma_{\sB = \sv}(T_R) \\
    %      ~~t: & p_R^{\sv}(
    %      \begin{array}[t]{@{}l}
    %        \iri_E(\sK_{RE}), \\
    %        \iri_F(\sK_{RF})) \}_{\sv \in \pi_{\sB} (T_R)}
    %      \end{array}
    %    \end{array}$
    %    & $\begin{array}{l}
    %         \{p_R^{\sv} \sqsubseteq p_R \}_{\sv \in \pi_{\sB} (T_R)}
    %       \end{array}$\\
    \bottomrule
  \end{tabularx}
}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/schema-driven-nopkey.tex <==
% Entity $E$ of attributes $\sA$ and primary identifier $\sK \subseteq \sA$
\begin{table}[t!]
  \caption{Schema-driven Patterns. For patterns yielding views, we show the views together with the DB schema, separating them from the original tables using a thick horizontal bar.}
  \label{tab:schema-driven-patterns}
  \centering
  {\linespread{0.96}\selectfont
  \resizebox{\textwidth}{!}{%
  \begin{tabularx}{1.5\textwidth}{lcXl@{}}
    \toprule
    \textsc{E-R diagram} & \textsc{DB schema} & \textsc{Mappings} & \textsc{Ontology}\\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Entity (SE/DE)}}\\
    \begin{minipage}{\erw}
      \centerline{\includegraphics[scale=\erscale]{img/er-SE.pdf}}
    \end{minipage}
    &
    % \begin{tabular}{l}
    %   \begin{tikzpicture}[dbpicture]
    %     \node (e) {$T_E(\pk{\sK},\sA)$};
    %   \end{tikzpicture}
    % \end{tabular}
    $T_E(\pk{\sK},\sA)$
    &
    $\begin{array}{l@{~}l}
      s{:} & T_E \\
      t{:} & C_E(\iri_E(\sK)), \\
           & \{d_A(\iri_E(\sK),A)\}_{A \in \sK\cup\sA}
    \end{array}$
    &
    $\begin{array}{l@{}}
      \{\exists d_A \sqsubseteq C_E \}_{A \in \sK\cup\sA}
    \end{array}$
    \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Relationship (SR/DR)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SR.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
              \sK\tikz\coordinate(kRF);_{RF}})$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
        s{:} & T_R \\
        t{:} & p_R(\iri_E(\sK_{RE}),\iri_F(\sK_{RF}))
      \end{array}$
    &
      $\begin{array}{l@{}}
        \exists p_R \sqsubseteq C_E \\
        \exists p_R^- \sqsubseteq C_F
       \end{array}$\\
       \multicolumn{4}{l}{\footnotesize
         In case of $(\_,1)$ cardinality on role $R_E$ (resp., $R_F$), the primary key for $T_R$ is restricted to the attributes $\sK_{RE}$ (resp., $\sK_{RF}$).
       } \\
       \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Relationship with Identifier Alignment
        (SRa/DRa)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRa.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK_F},\sU\tikz\coordinate(uF);_F,\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
              \sU\tikz\coordinate(kUF);_{RF}})$};
        \node[right=of r] (k) {$\key[R_F]{\sU_F}$};
        \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        \draw[->] ($(kUF)+(0,\uoffset)$) |- ($(kUF)+(0,\uuoffset)$) -|
          ($(uF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
%      s_1{:} & T_F \\
%      t_1{:} & C_F(\iri_F(\sK_F)), \\
%             & \{d_A(\iri_F(\sK_F),A) \\
%             & ~~\}_{A \in \sK_F\cup\sU_F\cup\sA_F}, \\[0.5ex]
      s{:} & T_R \Join_{\sU_{RF}=\sU_F} T_F\\
      t{:} & p_R(\iri_E(\sK_{RE}),\iri_F(\sK_F))
    \end{array}$
    &
    $\begin{array}{l@{}}
%      \{\exists d_A \sqsubseteq C_F \\
%      ~~\}_{A \in \sK_F\cup\sU_F\cup\sA_F} \\
      \exists p_R \sqsubseteq C_E \\
      \exists p_R^- \sqsubseteq C_F
     \end{array}$\\
     \multicolumn{4}{l}{\footnotesize
       In case of $(\_,1)$ cardinality on role $R_E$ (resp., $R_F$), the primary key for $T_R$ is restricted to the attributes $\sK_{RE}$ (resp., $\sU_{RF}$).
     } \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Relationship with Merging (SRm/DRm)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRm.pdf}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of f.south west,anchor=north west] (e)
          {$T_E(\pk{\sK_E},\sK\tikz\coordinate(kEF);_{EF},\sA_E)$};
        \draw[->] ($(kEF)+(0,\uoffset)$) |- ($(kEF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    & $\begin{array}{l@{~}l}
        s{:} & T_E \\
        t{:} & p_{EF}(\iri_E(\sK_E),\iri_F(\sK_{EF}))
      \end{array}$
    & $\begin{array}{l@{}}
        \exists p_{EF} \sqsubseteq C_E \\
        \exists p_{EF}^- \sqsubseteq C_F
      \end{array}$
    \\
    \midrule
    % \multicolumn{4}{c}{\textbf{Schema Entity with Weak Identification (SEw)}}\\
    % \begin{minipage}{\erw}
    %   \includegraphics[scale=\erscale]{img/er-SEw.pdf}
    % \end{minipage}
    % &
    % \begin{tabular}{l}
        %         \begin{tikzpicture}[dbpicture]
    %     \node (f)
    %       {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
    %     \node[below=of f.south west,anchor=north west] (e)
    %       {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kRF);_{RF}},\sA_E)$};
    %     \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
    %       ($(kF)-(0,\doffset)$);
    %   \end{tikzpicture}
    % \end{tabular}
    % &
    % $\begin{array}{l@{~}l}
    %   s{:} & T_E \\
    %   t{:} & C_E(\iri_E(\sK_E,\sK_{RF})), \\
    %        & \{ d_A(\iri_E(\sK_E,\sK_{RF}), A) \\
    %        & ~~\}_{A \in \sK_E \cup \sK_{RF} \cup \sA_E}, \\
    %        & p_R(\iri_E(\sK_E,\sK_{RF}),\iri_F(\sK_{RF}))
    % \end{array}$
    % &
    % $\begin{array}{l@{}}
    %   \{\exists d_A \sqsubseteq C_E \\
    %   ~~\}_{A \in \sK_E\cup\sA_E} \\
    %   \exists p_R \sqsubseteq C_E \\
    %   \exists p_R^- \sqsubseteq C_F
    % \end{array}$\\
    % \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Reified Relationship (SRR/DRR)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SRR.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      $\sK_R:=\sK_{RE}\cup\sK_{RF}\cup\sK_{RG}$\\
      \begin{tikzpicture}[dbpicture]
        \node (g)
          {$T_G(\pk{\sK\tikz\coordinate(kG);_G},\sA_G)$};
        \node[below=of g] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
            \sK\tikz\coordinate(kRF);_{RF},
            \sK\tikz\coordinate(kRG);_{RG}},
           \sA_R)$};
        \node[below=of r.south west,anchor=north west] (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \draw[->] ($(kRE)-(0,\doffset)$) -- ($(kE)+(0,\uoffset)$);
        \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
          ($(kF)+(0,\uoffset)$);
        \draw[->] ($(kRG)+(0,\uoffset)$) |- ($(kRG)+(0,\uuoffset)$) -|
          ($(kG)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
    $\begin{array}{l@{~}l}
      s{:} & T_R\\
      t{:} & C_R(\iri_R(\sK_R)), \\
      %    & \{d_A(\iri_R(\sK_R), A)\}_{A \in \atts(T_R)}, \\
           & \{d_A(\iri_R(\sK_R), A)\}_{A \in \sK_R\cup\sA_R}, \\
           & p_{RE}(\iri_R(\sK_R), \iri_E(\sK_{RE})), \\
           & p_{RF}(\iri_R(\sK_R), \iri_F(\sK_{RF})), \\
           & p_{RG}(\iri_R(\sK_R), \iri_G(\sK_{RG}))
    \end{array}$
    &
    $\begin{array}{l@{}}
      \exists p_{RE} \sqsubseteq C_R \\
      \exists p_{RE}^- \sqsubseteq C_E \\
      \exists p_{RF} \sqsubseteq C_R \\
      \exists p_{RF}^- \sqsubseteq C_F \\
      \exists p_{RG} \sqsubseteq C_R \\
      \exists p_{RG}^- \sqsubseteq C_G \\
      \{\exists d_A \sqsubseteq C_R\}_{A \in \sK_R\cup\sA_R}
     \end{array}$\\[9ex]
     \multicolumn{4}{l}{\footnotesize
       \begin{minipage}{1.48\linewidth}
         \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
         

         \pat{SRR} applies whenever there are three or more participating roles, or when the relationship has attributes. If $R$ is identified by a strict subset $X$ of the participating roles, then the primary key of table $T_R$ (and the corresponding set of attributes $\sK_R$) is restricted to the foreign keys corresponding to the roles in $X$. For instance, if $R$ is identified by roles $R_E$ and $R_G$, then the primary key of $T_R$ (and the corresponding set of attributes $\sK_R$) is $\sK_{RE} \cup \sK_{RG}$. If one of the foreign keys is to a non-primary key set of attributes, the object property relative to that foreign key is dealt with as in \pat{SRa}.
       \end{minipage}
   } \\
     \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Hierarchy (SH/DH)}}\\
    \begin{minipage}{\erw}
      \centerline{\includegraphics[scale=\erscale]{img/er-SH.pdf}}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_{FE}},\sA_F)$};
        \draw[->] ($(kF)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
        s{:} & T_F \\
        t{:} & C_F(\iri_E(\sK_{FE})), \\
             & \{d_A(\iri_E(\sK_{FE}),A)\}_{A \in \sA_F}
       \end{array}$
    &
      $\begin{array}{l@{}}
         C_F \sqsubseteq C_E \\
         \{\exists d_A \sqsubseteq C_F \}_{A \in \sA_F}
      \end{array}$
      \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema/Data Hierarchy with Identifier Alignment (SHa/DHa)}}\\
    \begin{minipage}{\erw}
      \centering
      \includegraphics[scale=\erscale]{img/er-SHa.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sU\tikz\coordinate(uF);_F,
           \sA_F)$};
        \node[below=of e.east,anchor=west] (k)
          {$\key[T_F]{\sU_F}$};
        \draw[->] ($(uF)+(0,\uoffset)$) |- ($(uF)+(0,\uuoffset)$) -|
          ($(kE)-(0,\doffset)$);
        \end{tikzpicture} \\
      \bottomrule
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
          {$V_F(\sK\tikz\coordinate(kF);_F,\pk{\sU\tikz\coordinate(uF);_F},
            \sA_F) = T_F$ };
        \node[right=of e.east,anchor=west] (k)
          {$\key[V_F]{\sK_F}$ };
        \draw[->] ($(uF)+(0,\uoffset)$) |- ($(uF)+(0,\uuoffset)$) -|
          ($(kE)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
         s{:} & T_F \\
         t{:} & C_F(\iri_E(\sU_F)), \\[0.5ex]
         & \{d_A(\iri_E(\sU_F),A)\}_{A \in \sK_F \cup \sA_F}
      \end{array}$
    &
      $\begin{array}{l@{}}
        C_F \sqsubseteq C_E \\
         \{\exists d_A \sqsubseteq C_F \}_{A \in \sK_F\cup\sA_F}
    \end{array}$
    \\
    \multicolumn{4}{l}{\footnotesize
      \begin{minipage}{1.48\linewidth}
         \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
        In this pattern, the ``alignment'' is meant to align the primary identifier used in the child entity to the primary identifier used in the parent entity. We here depict the most common scenario, where the foreign key points to the primary key of the parent entity. The other two possiblities for the application of the pattern are:

        \begin{compactitem}
        \item the foreign key in the child entity coincides with the primary key of that entity, and references a non-primary key of the parent entity;
        \item the foreign key in the child entity does not coincide with the primary key of that entity, and  references a non-primary key of the parent entity.
        \end{compactitem}
      \end{minipage}
    }\\
    % \midrule
    % \multicolumn{4}{c}{\textbf{Schema/Data Hierarchy with Advanced Alignment (SHaa/DHaa)}}\\
    % \begin{minipage}{\erw}
    %   \begin{center}
    %      \includegraphics[scale=\erscale]{img/er-SHaa.pdf}\\
    %      {\footnotesize $\sK_{E}$ in $F$ is a constant \texttt{c},\\[-.5ex]
    %        $\sK_{EF}$ alone identifies $F$.
    %      }
    %    \end{center}
    %  \end{minipage}
    %  &
    %  \begin{tabular}{l}
    %    \begin{tikzpicture}[dbpicture]
    %      \node (e)
    %        {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kEF);_{EF}},\sA_E)$};
    %      \node[below=of e.south west,anchor=north west] (f)
    %      {$T_F(\pk{\sK\tikz\coordinate(kF);_{F}},\sA_F)$};
    %      \draw[->, dashed] ($(kF)+(0,\uoffset)$) |- ($(kF)+(0,\uuoffset)$) -| ($(kEF)-(0,\doffset)$);
    %    \end{tikzpicture}
    %  \end{tabular}
    %  &
    %    $\begin{array}{l@{~}l}
    %      s{:} & \pi_{\texttt{c}, \sK_{F}}(T_F) \\
    %      t{:} & C_F(\iri_E(\texttt{c}, \sK_{F})), \\
    %           & \{d_A(\iri_E(\texttt{c},\sK_{F}),A)\}_{A \in \sA_F}
    %     \end{array}$
    %  &
    %    $\begin{array}{l@{}}
    %       C_F \sqsubseteq C_E \\
    %       \{\exists d_A \sqsubseteq C_F \}_{A \in \sA_F}
    %    \end{array}$
    %    \\~\\[-1ex]
    %    \multicolumn{4}{l}{\footnotesize
    %    \begin{minipage}{1.48\linewidth}
    %      $\sK_{E}$ is not inherited by the child table, because it is a constant value \texttt{c}. The dependency between $T_F$ and $T_E$ is an inclusion dependency, rather than a foreign key dependency.
    %    \end{minipage}
    %  }\\
    \bottomrule
  \end{tabularx}
}
}
\end{table}


%%% Discarded
\endinput

\begin{table}[t!]
  \caption{Schema-driven Patterns for Hierarchies}
  \label{tab:schema-driven-patterns-hierarchies}
 \resizebox{\textwidth}{!}{
  \begin{tabularx}{1.15\textwidth}{lcXl@{}}
    \toprule
    \textsc{E-R diagram} & \textsc{DB schema} & \textsc{Mapping pattern} & \textsc{Ontology}
    \\
    \midrule
    \multicolumn{4}{c}{\textbf{Schema Hierarchy with Identifier Alignment (SHa)\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SHa.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      $\sK_R:=\sK_{RF}\cup\sK_{RG}$\\
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sU\tikz\coordinate(uF);_F,
           \sA_F)$};
        \node[right=of e] (g)
          {$T_G(\pk{\sK\tikz\coordinate(kG);_G},\sA_G)$};
        \node[below=of f.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRF);_{RF},
              \sK\tikz\coordinate(kRG);_{RG}},
             \sA_R)$};
        \node[below=of r.south west,anchor=north west] (k)
          {$\key[T_F]{\sU_F}$};
        \draw[->] ($(uF)+(0,\uoffset)$) |- ($(uF)+(0,\uuoffset)$) -|
          ($(kE)-(0,\doffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) -- ($(kF)-(0,\doffset)$);
        \draw[->] ($(kRG)+(0,\uoffset)$) |- ($(kRG)+(0,\uuoffset)$) -|
          ($(kG)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
    &
      $\begin{array}{l@{~}l}
        s_1{:} & T_R \\
        t_1{:} & C_R(\iri_R(\sK_R)), \\
               & \{
               \begin{array}[t]{@{}l}
                 d_A(\iri_R(\sK_R),A)\\
                 \}_{A \in \sK_R\cup\sA_R},
               \end{array} \\
               & p_{RG}(\iri_R(\sK_R), \iri_G(\sK_{RG})) \\[0.5ex]
        s_2{:} & T_F \\
        t_2{:} & C_F(\iri_E(\sU_F)) \\[0.5ex]
        s_3{:} & T_R \Join_{\sK_{RF}=\sK_F} T_F \\
        t_3{:} & p_{RF}(\iri_R(\sK_R), \iri_E(\sU_F))
      \end{array}$
    &
      $\begin{array}{l@{}}
        C_F \sqsubseteq C_E \\
        \exists p_{RF} \sqsubseteq C_R \\
        \exists p_{RF}^- \sqsubseteq C_F \\
        \exists p_{RG} \sqsubseteq C_R \\
        \exists p_{RG}^- \sqsubseteq C_G \\
        \{\exists d_A^- \sqsubseteq C_R \}_{A \in \sK_R\cup\sA_R}
    \end{array}$
    \\
    \bottomrule
  \end{tabularx}
}
\end{table}

==> tables/schema-normalization.tex <==
% Entity $E$ of attributes $\sA$ and primary identifier $\sK \subseteq \sA$
\begin{table}[t!]
  \caption{Schema-normalization Functions. We assume the input DB to be at least 1st NF. Depending on how we apply the BCNF operator, we \emph{might} end-up in a BCNF.}
  \label{tab:schema-normalization}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccc}
    \toprule
    \textsc{E-R diagram} & \textsc{DB schema} & \textsc{Output Schema} \\
    \midrule
    \multicolumn{3}{c}{\textbf{Key Alignment}}\\
    \begin{minipage}{\erw}
      \centering
      \includegraphics[scale=\erscale]{img/er-SHa.pdf}
    \end{minipage}
    &
    \begin{tikzpicture}[dbpicture]
      \node (e)
      {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
      \node[below=of e.south west,anchor=north west] (f)
      {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sU\tikz\coordinate(uF);_F,
          \sA_F)$};
      \node[below=of e.east,anchor=west] (k)
      {$\key[T_F]{\sU_F}$};
      \draw[->] ($(uF)+(0,\uoffset)$) |- ($(uF)+(0,\uuoffset)$) -|
      ($(kE)-(0,\doffset)$);
    \end{tikzpicture}
    &
    \begin{tikzpicture}[dbpicture]
        \node (e)
        {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
        {$V_F(\sK\tikz\coordinate(kF);_F,\pk{\sU\tikz\coordinate(uF);_F},
          \sA_F) := T_F$};
        \node[right=of e.east,anchor=west] (k)
        {$\key[V_F]{\sK_F}$ };
        \draw[->] ($(uF)+(0,\uoffset)$) |- ($(uF)+(0,\uuoffset)$) -|
        ($(kE)-(0,\doffset)$);
      \end{tikzpicture}
      \\
    \multicolumn{3}{l}{\footnotesize
    \begin{minipage}{1.4\linewidth}
      \setdefaultleftmargin{1em}{0em}{0em}{0em}{0em}{0em}
        In this pattern, the ``alignment'' is meant to align the primary identifier used in the child entity to the primary identifier used in the parent entity. We here depict the most common scenario, where the foreign key points to the primary key of the parent entity. The other two possiblities for the application of the pattern are:
        \begin{compactitem}
        \item the foreign key in the child entity coincides with the primary key of that entity, and references a non-primary key of the parent entity;
        \item the foreign key in the child entity does not coincide with the primary key of that entity, and  references a non-primary key of the parent entity.
        \end{compactitem}
      \end{minipage}
    }\\
    \midrule
    \multicolumn{3}{c}{\textbf{Key Completion}}\\
    \begin{minipage}{\erw}
      \begin{center}
        \includegraphics[scale=\erscale]{img/er-SHaa.pdf}\\
        {\footnotesize $\sK_{E}$ in $F$ is a tuple of constants $\vec{c_F}$,\\[-.5ex]
          $\sK_{EF}$ alone identifies $F$.
        }
      \end{center}
    \end{minipage}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK_E,\sK\tikz\coordinate(kEF);_{EF}},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
        {$T_F(\pk{\sK\tikz\coordinate(kF);_{F}},\sA_F)$};
        \draw[->,dashed] ($(kF)+(0,\uoffset)$) |- ($(kF)+(0,\uuoffset)$) -| ($(kEF)-(0,\doffset)$);
      \end{tikzpicture}\\
      {\footnotesize
      \begin{tabular}{l}
        For every tuple $v$ in $\sK_{F}$, \\
        there is a tuple $(\vec{c_F},\vec{v})$ in $(\sK_{E}, \sK_{EF})$,\\
        where $\vec{c_F}$ is a tuple of constants.
      \end{tabular}
      }
    \end{tabular}
    &
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (e)
        {$T_E(\pk{\sK_E,\tikz\coordinate(kEF);\sK_{EF}},\sA_E)$};
        \node[below=of e.south west,anchor=north west] (f)
        {$V_F(\pk{\sK_E\tikz\coordinate(kF);,\sK_{F}},\sA_F) := \pi_{\texttt{\textbf{c}}, \sK_{F}}(T_F)$};
        \draw[->] ($(kF)+(0,\uoffset)$) |- ($(kF)+(0,\uuoffset)$) -| ($(kEF)-(0,\doffset)$);
      \end{tikzpicture}
    \end{tabular}
      \\~\\[-1ex]
      \multicolumn{3}{l}{\footnotesize
      \begin{minipage}{1.4\linewidth}
        $\sK_{E}$ is not inherited by the child table, because it is a tuple of constant values $\vec{c_F}$. The dashed arrow between $T_F$ and $T_E$ denotes an inclusion dependency.
      \end{minipage}
    }\\
    \midrule
    \multicolumn{3}{c}{\textbf{3NF operator 1 (Data-Lossless Vertical Decomposition)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR1Nm.pdf}
    \end{minipage} &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
         T_E(\pk{\sK_E},\sA_E,\sK_F,\sA_F)\\[1ex]
         \fd[T_E]{\sK_F}{\sA_F}\\
       \end{array}$
    \end{tabular}&
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (ve)
        {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) = \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of ve.south west,anchor=north west] (vr)
        {$V_R(\pk{\sK\tikz\coordinate(kRE);_E},\sK\tikz\coordinate(kRF);_F) =
           \pi_{\sK_E,\sK_F} (T_E)$};
         \node[below=of vr.south west,anchor=north west] (vf)
         {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
         \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
         \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
         ($(kF)+(0,\uoffset)$);
       \end{tikzpicture}
    \end{tabular}\\
    \midrule
    \multicolumn{3}{c}{\textbf{3NF operator 2 (Data-Lossless Vertical Decomposition)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DR1Nm.pdf}
    \end{minipage} &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
         T_E(\pk{\sK_E},\sA_E,\sK_F,\sA_F)\\[1ex]
         \fd[T_E]{\sK_F}{\sA_F}\\
       \end{array}$
    \end{tabular}&
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (vf)
        {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \node[below=of vf.south west,anchor=north west] (ve)
        {$V_E(\pk{\sK_E}, \sK\tikz\coordinate(kF2);_F, \sA_E) = \pi_{\sK_E,\sK_F,\sA_E} (T_E)$};
        \draw[->] ($(kF2)+(0,\uoffset)$) |- ($(kF)-(0,\uuoffset)$) |- ($(kF)-(0,\doffset)$);        
%         \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
 %        ($(kF)+(0,\uoffset)$);
       \end{tikzpicture}
    \end{tabular}\\
    \midrule
    \multicolumn{3}{c}{\textbf{2NF Operator 1 (Data-Lossless Vertical Decomposition)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SEw.pdf}
    \end{minipage} &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
         T_E(\pk{\sK_E,\sK_F},\sA_E,\sA_F)\\[1ex]
         \fd[T_E]{\sK_F}{\sA_F}\\
       \end{array}$
    \end{tabular}&
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
        \node (ve)
        {$V_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E) = \pi_{\sK_E,\sA_E} (T_E)$};
        \node[below=of ve.south west,anchor=north west] (vr)
        {$V_R(\pk{\sK\tikz\coordinate(kRE);_E},\sK\tikz\coordinate(kRF);_F) =
           \pi_{\sK_E,\sK_F} (T_E)$};
         \node[below=of vr.south west,anchor=north west] (vf)
         {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
         \draw[->] ($(kRE)+(0,\uoffset)$) -- ($(kE)-(0,\doffset)$);
         \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
         ($(kF)+(0,\uoffset)$);
       \end{tikzpicture}
    \end{tabular}\\
    \midrule
        \multicolumn{3}{c}{\textbf{2NF Operator 2 (Data-Lossless Vertical Decomposition)}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-SEw.pdf}
    \end{minipage} &
    \begin{tabular}{@{}l@{}}
      $\begin{array}{@{~}l}
         T_E(\pk{\sK_E,\sK_F},\sA_E,\sA_F)\\[1ex]
         \fd[T_E]{\sK_F}{\sA_F}\\
       \end{array}$
    \end{tabular}&
    \begin{tabular}{l}
      \begin{tikzpicture}[dbpicture]
                \node (vf)
        {$V_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F) = \pi_{\sK_F,\sA_F} (T_E)$};
        \node[below=of vf.south west,anchor=north west] (ve)
        {$V_E(\pk{\sK_E}, \sK\tikz\coordinate(kF2);_F, \sA_E) = \pi_{\sK_E,\sK_F,\sA_E} (T_E)$};
        \draw[->] ($(kF2)+(0,\uoffset)$) |- ($(kF)-(0,\uuoffset)$) |- ($(kF)-(0,\doffset)$);        
%         \draw[->] ($(kRF)-(0,\doffset)$) |- ($(kRF)-(0,\ddoffset)$) -|
 %        ($(kF)+(0,\uoffset)$);
       \end{tikzpicture}
    \end{tabular}\\
    \midrule
    \multicolumn{3}{c}{\textbf{Role-introduction (RI) operator}}\\
    \begin{minipage}{\erw}
      \includegraphics[scale=\erscale]{img/er-DH01.pdf}
    \end{minipage}
    &
    \begin{tabular}{@{}l@{}}
      \begin{tikzpicture}[dbpicture]
        \node (e)
          {$T_E(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
          {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
            \sK\tikz\coordinate(kRF);_{RF}})$};
        \draw[->] ($(kRE)+(0.3mm,\uoffset)$) -- ($(kE)-(0,\doffset)$);
        % \draw[->] ($(kSG)-(0,\doffset)$) |- ($(kSG)-(0,\ddoffset)$) -|
        %  ($(kG)+(0,\uoffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
        \end{tikzpicture}\\
      \end{tabular}&
      \begin{tabular}{l}
        \begin{tikzpicture}[dbpicture]
        \node (e0)
          {$T_E(\pk{\sK\tikz\coordinate(kE0);_E},\sA_E)$};
        \node[below=of e0.south west,anchor=north west] (e)
          {$V_{E_R}(\pk{\sK\tikz\coordinate(kE);_E},\sA_E)$};
        \node[right=of e] (f)
          {$T_F(\pk{\sK\tikz\coordinate(kF);_F},\sA_F)$};
        \node[below=of e.south west,anchor=north west] (r)
        {$T_R(\pk{\sK\tikz\coordinate(kRE);_{RE},
            \sK\tikz\coordinate(kRF);_{RF}})$};
        \draw[->] ($(kE)+(0.3mm,\uoffset)$) |- ($(kE0)-(0,\uuoffset)$) |- ($(kE0)-(0,\doffset)$);
        \draw[->] ($(kRE)+(0.3mm,\uoffset)$) |- ($(kE)-(0,\uuoffset)$) |- ($(kE)-(0,\doffset)$);
        % \draw[->] ($(kSG)-(0,\doffset)$) |- ($(kSG)-(0,\ddoffset)$) -|
        %  ($(kG)+(0,\uoffset)$);
        \draw[->] ($(kRF)+(0,\uoffset)$) |- ($(kRF)+(0,\uuoffset)$) -|
          ($(kF)-(0,\doffset)$);
        \end{tikzpicture}\\
        where\\
        $\begin{array}{l}
         V_{E_R}(\sK_E,\sA_E) ={}\\
         \quad \pi_{\sK_E,\sA_E}(T_R \Join_{\sK_{RE}=\sK_E} T_E)
       \end{array}$
      \end{tabular}\\
    \midrule
    \multicolumn{3}{c}{\textbf{Entity Clustering (EC) (Horizontal Decomposition)}}\\
    \begin{minipage}{\erw}
      \begin{center}
        \includegraphics[scale=\erscale]{img/er-SE.pdf}
        \smallskip
        $\begin{array}{c}
           \sB \subseteq \sK\cup\sA,\\
           \partition_\D(\sB,E)
         \end{array}
         $
       \end{center}
     \end{minipage}
                         & $\begin{array}{l}
                              T_E(\pk{\sK}, \sA) \\
                              \sB \subseteq \sK\cup\sA \\
                              \partition_\D(\sB,E) \\
                            \end{array}$
                         & \begin{minipage}{\erw}
                           \begin{tikzpicture}[dbpicture]
                             \node (e) {$T_E(\pk{\sK\tikz\coordinate(K);}, \sA)$} ;
                             \node[below=of e.south west,anchor=north west] (v) {
                               $\begin{array}{l}
                                  \{V_{E_{\sv}}(\pk{\sK}\tikz\coordinate(KV);,\sA) = \\ \quad \sigma_{\sB = \sv}(T_E)\}_{\sv \in \pi_{\sB} (T_E)}
                                \end{array}$} ;
                              \draw[->] ($(KV)+(-1mm,\uoffset)$) |- ($(K)-(0,\uuoffset)$) -|
                              ($(K)-(1mm,\doffset)$);
                            \end{tikzpicture}
                            \end{minipage}\\
    \multicolumn{3}{l}{\footnotesize
    \begin{minipage}{1.4\linewidth}
      $\sK_{E}$ is not inherited by the child table, because it is a tuple of constant values \texttt{\textbf{c}}. The dashed arrow between $T_F$ and $T_E$ denotes an inclusion dependency.
    \end{minipage}
    }\\
    % \midrule
    % \multicolumn{3}{c}{\textbf{Relationship Clustering (RC) (Horizontal Decomposition)}}\\
    %     \begin{minipage}{\erw}
    %       \begin{center}
    %     \includegraphics[scale=\erscale]{img/er-CR2O.pdf}
    %     \smallskip
    %     $\begin{array}{c}
    %        \sB \subseteq \sK_{RE}\cup\sK_{RF},\\
    %        \partition_\D(\sB,R)
    %     \end{array}
    %     $
    %   \end{center}
    % \end{minipage}
    % & $\begin{array}{l}
    %      T_R(\sK_{RE},\sK_{RF}), \\
    %      \sB \subseteq \sK_{RE}\cup\sK_{RF}\\
    %      \partition_\D(\sB,R) \\
    %    \end{array}$
    %    &
    %      \textcolor{red}{TODO: Like above}
    %      $\begin{array}{l}
    %      \{V_{R_{\sv}}(\sK_{RE},\sK_{RF}) = \\
    %      \quad \sigma_{\sB = \sv}(T_R)\}_{\sv \in \pi_{\sB} (T_R)}
    %    \end{array}$
    %    \\
       \bottomrule
     \end{tabular}
}
\end{table}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

